Abstract structure of unitary oracles for quantum algorithms

We show that a pair of complementary dagger-Frobenius algebras, equipped with a self-conjugate comonoid homomorphism onto one of the algebras, produce a nontrivial unitary morphism on the product of the algebras. This gives an abstract understanding of the structure of an oracle in a quantum computation, and we apply this understanding to develop a new algorithm for the deterministic identification of group homomorphisms into abelian groups. We also discuss an application to the categorical theory of signal-flow networks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{270}
\providecommand{\publicationstatus}{B. Coecke, I. Hasuo \& P. Panangaden (Eds.):\\
Quantum Physics and Logic 2014 (QPL 2014).\\
EPTCS 172, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.172.19}{10.4204/EPTCS.172.19}}

